Parsing with Pretrained Language Models, Multiple Datasets, and Dataset Embeddings

With an increase of dataset availability, the potential for learning from a variety of data sources has increased. One particular method to improve learning from multiple data sources is to embed the data source during training. This allows the model to learn generalizable features as well as distinguishing features between datasets. However, these dataset embeddings have mostly been used before contextualized transformer-based embeddings were introduced in the field of Natural Language Processing. In this work, we compare two methods to embed datasets in a transformer-based multilingual dependency parser, and perform an extensive evaluation. We show that: 1) embedding the dataset is still beneficial with these models 2) performance increases are highest when embedding the dataset at the encoder level 3) unsurprisingly, we confirm that performance increases are highest for small datasets and datasets with a low baseline score. 4) we show that training on the combination of all datasets performs similarly to designing smaller clusters based on language-relatedness.

==> table-1.tex <==
\begin{table}[hbtp!]
  \small
\begin{tabular}{ll|rrrrrr}
  cluster                    & treebank                     & \multicolumn{1}{l}{\textsc{m} } & \multicolumn{1}{l}{\textsc{c} } & \multicolumn{1}{l}{\textsc{dd}} & \multicolumn{1}{l}{\textsc{de}} & \multicolumn{1}{l}{$\delta$ \textsc{dd}-max(\textsc{m},\textsc{c})} & \multicolumn{1}{l}{$\delta$ \textsc{de}-max(\textsc{m},\textsc{c})} \\
\toprule
         & Dutch-Alpino                 & 92.7                         & 93.0                           & \textbf{93.2}                         & 92.8                                  & \cellcolor[HTML]{F9FDFB}0.2                & \cellcolor[HTML]{FDF4F4}-0.2               \\
                           & Dutch-LassySmall             & 86.7                         & 89.4                           & \textbf{89.6}                         & 89.3                                  & \cellcolor[HTML]{F9FDFB}0.2                & \cellcolor[HTML]{FEF9F9}-0.1               \\
\multirow{-3}{*}{af-de-nl} & German-GSD                   & 88.0                         & 88.5                           & \textbf{88.6}                         & 88.4                                  & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{FEF9F9}-0.1               \\
                           \midrule
                           & Russian-SynTagRus            & 94.3                         & 94.3                           & \textbf{94.4}                         & 94.3                                  & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{FFFFFF}0.0                \\
                           & Russian-Taiga                & \textbf{76.9}                & 76.2                           & 76.6                                  & \textbf{77.5}                         & \cellcolor[HTML]{FCEFEE}-0.3               & \cellcolor[HTML]{EDF8F3}0.6                \\
\multirow{-3}{*}{e-sla}    & Ukrainian-IU                 & 87.6                         & 88.9                           & \textbf{89.0}                         & 88.5                                  & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{FBEAE9}-0.4               \\
                           \midrule
                           & English-EWT                  & \textbf{89.1}                & 88.3                           & 88.8                                  & 88.9                                  & \cellcolor[HTML]{FCEFEE}-0.3               & \cellcolor[HTML]{FDF4F4}-0.2               \\
                           & English-GUM                  & \textbf{89.9}                & 88.1                           & \textbf{89.9}                         & \textbf{90.4}                         & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{F0F9F5}0.5                \\
\multirow{-3}{*}{en}       & English-LinES                & \textbf{86.6}                & 84.0                           & 85.3                                  & \textbf{87.4}                         & \cellcolor[HTML]{F2BDB9}-1.3               & \cellcolor[HTML]{E7F6EE}0.8                \\
                           \midrule
                           & Catalan-AnCora               & 93.1                         & \textbf{93.5}                  & 93.4                                  & 93.4                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{FEF9F9}-0.1               \\
\multirow{-2}{*}{es-ca}    & Spanish-AnCora               & 92.8                         & \textbf{93.1}                  & \textbf{93.1}                         & 93.0                                  & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{FEF9F9}-0.1               \\
                           \midrule
                           & Estonian-EDT                 & \textbf{85.9}                & 85.6                           & 85.7                                  & 85.6                                  & \cellcolor[HTML]{FDF4F4}-0.2               & \cellcolor[HTML]{FCEFEE}-0.3               \\
                           & Finnish-FTB                  & 88.5                         & 81.6                           & \textbf{89.1}                         & \textbf{89.8}                         & \cellcolor[HTML]{EDF8F3}0.6                & \cellcolor[HTML]{D8EFE4}1.3                \\
                           & Finnish-TDT                  & 88.6                         & 83.4                           & \textbf{89.2}                         & \textbf{89.4}                         & \cellcolor[HTML]{EDF8F3}0.6                & \cellcolor[HTML]{E7F6EE}0.8                \\
\multirow{-4}{*}{finno}    & North\_Sami-Giella           & 33.3                         & 42.0                           & \textbf{42.2}                         & \textbf{44.2}                         & \cellcolor[HTML]{F9FDFB}0.2                & \cellcolor[HTML]{BCE4D1}2.2                \\
                           \midrule
                           & French-Sequoia               & 83.4                         & 84.6                           & \textbf{86.2}                         & \textbf{90.1}                         & \cellcolor[HTML]{CFECDD}1.6                & \cellcolor[HTML]{57BB8A}5.5                \\
\multirow{-2}{*}{fr}       & French-Spoken                & 37.0                         & 72.9                           & \textbf{73.3}                         & \textbf{74.0}                         & \cellcolor[HTML]{F3FBF7}0.4                & \cellcolor[HTML]{DEF2E8}1.1                \\
                           \midrule
                           & Hindi-HDTB                   & 92.4                         & 92.3                           & \textbf{92.5}                         & 92.4                                  & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{FFFFFF}0.0                \\
\multirow{-2}{*}{indic}    & Urdu-UDTB                    & 80.1                         & \textbf{81.2}                  & 81.0                                  & 81.1                                  & \cellcolor[HTML]{FDF4F4}-0.2               & \cellcolor[HTML]{FEF9F9}-0.1               \\
                           \midrule
                           & Italian-ISDT                 & 92.9                         & 92.9                           & \textbf{93.1}                         & 92.9                                  & \cellcolor[HTML]{F9FDFB}0.2                & \cellcolor[HTML]{FFFFFF}0.0                \\
\multirow{-2}{*}{it}       & Italian-PoSTWITA             & 79.2                         & \textbf{80.6}                  & 80.2                                  & 80.1                                  & \cellcolor[HTML]{FBEAE9}-0.4               & \cellcolor[HTML]{FAE5E4}-0.5               \\
                           \midrule
                           & Korean-GSD                   & \textbf{82.4}                & 70.7                           & 79.8                                  & 82.1                                  & \cellcolor[HTML]{E67C73}-2.6               & \cellcolor[HTML]{FCEFEE}-0.3               \\
\multirow{-2}{*}{ko}       & Korean-Kaist                 & \textbf{87.4}                & 83.3                           & 87.1                                  & 87.2                                  & \cellcolor[HTML]{FCEFEE}-0.3               & \cellcolor[HTML]{FDF4F4}-0.2               \\
                           \midrule
                           & Danish-DDT                   & 85.2                         & \textbf{85.7}                  & 85.6                                  & \textbf{86.1}                         & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{F3FBF7}0.4                \\
                           & Norwegian-Bokmaal            & 93.2                         & \textbf{94.0}                  & 93.9                                  & \textbf{94.1}                         & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{FCFEFD}0.1                \\
                           & Norwegian-Nynorsk            & 91.7                         & 92.7                           & \textbf{92.9}                         & \textbf{93.0}                         & \cellcolor[HTML]{F9FDFB}0.2                & \cellcolor[HTML]{F6FCF9}0.3                \\
                           & Norwegian-NynorskLIA         & 71.6                         & \textbf{74.2}                  & 74.0                                  & \textbf{74.9}                         & \cellcolor[HTML]{FDF4F4}-0.2               & \cellcolor[HTML]{EAF7F1}0.7                \\
                           & Swedish-LinES                & 84.6                         & 85.2                           & \textbf{85.7}                         & \textbf{86.0}                         & \cellcolor[HTML]{F0F9F5}0.5                & \cellcolor[HTML]{E7F6EE}0.8                \\
\multirow{-6}{*}{n-ger}    & Swedish-Talbanken            & 83.2                         & 83.6                           & \textbf{84.5}                         & \textbf{85.0}                         & \cellcolor[HTML]{E4F4EC}0.9                & \cellcolor[HTML]{D5EEE2}1.4                \\
                           \midrule
                           & Ancient\_Greek-Perseus       & 58.9                         & \textbf{64.5}                  & 64.2                                  & 63.7                                  & \cellcolor[HTML]{FCEFEE}-0.3               & \cellcolor[HTML]{F7D6D3}-0.8               \\
                           & Ancient\_Greek-PROIEL        & 72.1                         & \textbf{75.4}                  & 74.9                                  & 74.5                                  & \cellcolor[HTML]{FAE5E4}-0.5               & \cellcolor[HTML]{F6D1CE}-0.9               \\
                           & Gothic-PROIEL                & 70.3                         & \textbf{78.1}                  & \textbf{78.1}                         & 77.4                                  & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{F8DBD9}-0.7               \\
                           & Latin-ITTB                   & 89.7                         & \textbf{89.9}                  & \textbf{89.9}                         & \textbf{90.0}                         & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{FCFEFD}0.1                \\
                           & Latin-PROIEL                 & 79.7                         & \textbf{81.4}                  & 81.3                                  & 80.6                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{F7D6D3}-0.8               \\
\multirow{-6}{*}{old}      & Old\_Church\_Slavonic-PROIEL & 62.1                         & \textbf{65.6}                  & 65.5                                  & 64.8                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{F7D6D3}-0.8               \\
                           \midrule
                           & Galician-CTG                 & 79.9                         & \textbf{80.3}                  & \textbf{80.3}                         & \textbf{80.3}                         & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{FFFFFF}0.0                \\
\multirow{-2}{*}{pt-gl}    & Portuguese-Bosque            & 90.3                         & 90.2                           & \textbf{90.4}                         & 90.2                                  & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{FEF9F9}-0.1               \\
\midrule
                           & Croatian-SET                 & 88.5                         & 88.6                           & \textbf{88.9}                         & 88.8                                  & \cellcolor[HTML]{F6FCF9}0.3                & \cellcolor[HTML]{F9FDFB}0.2                \\
                           & Serbian-SET                  & 86.1                         & 86.9                           & \textbf{88.3}                         & 87.9                                  & \cellcolor[HTML]{D5EEE2}1.4                & \cellcolor[HTML]{E1F3EA}1.0                \\
                           & Slovenian-SSJ                & 92.8                         & \textbf{93.4}                  & \textbf{93.4}                         & 93.2                                  & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{FDF4F4}-0.2               \\
\multirow{-4}{*}{sw-sla}   & Slovenian-SST                & 23.5                         & 63.1                           & \textbf{63.8}                         & 61.8                                  & \cellcolor[HTML]{EAF7F1}0.7                & \cellcolor[HTML]{F2BDB9}-1.3               \\
                           \midrule
                           & Turkish-IMST                 & \textbf{64.6}                & \textbf{64.6}                  & 64.5                                  & 64.4                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{FDF4F4}-0.2               \\
\multirow{-2}{*}{turkic}   & Uyghur-UDT                   & 41.2                         & \textbf{45.0}                  & \textbf{45.0}                         & 44.0                                  & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{F5CCC9}-1.0               \\
                           \midrule
                           & Czech-CAC                    & 91.9                         & \textbf{92.6}                  & 92.5                                  & 92.3                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{FCEFEE}-0.3               \\
                           & Czech-FicTree                & 92.8                         & 93.5                           & \textbf{93.6}                         & \textbf{94.0}                         & \cellcolor[HTML]{FCFEFD}0.1                & \cellcolor[HTML]{F0F9F5}0.5                \\
                           & Czech-PDT                    & 90.4                         & 91.0                           & \textbf{91.3}                         & 91.1                                  & \cellcolor[HTML]{F6FCF9}0.3                & \cellcolor[HTML]{FCFEFD}0.1                \\
                           & Polish-LFG                   & 95.2                         & 93.4                           & \textbf{95.9}                         & \textbf{96.3}                         & \cellcolor[HTML]{EAF7F1}0.7                & \cellcolor[HTML]{DEF2E8}1.1                \\
                           & Polish-PDB                   & \textbf{91.2}                & 90.9                           & \textbf{91.2}                         & 91.1                                  & \cellcolor[HTML]{FFFFFF}0.0                & \cellcolor[HTML]{FEF9F9}-0.1               \\
\multirow{-6}{*}{w-sla}    & Slovak-SNK                   & 92.0                         & \textbf{93.6}                  & 93.5                                  & 93.5                                  & \cellcolor[HTML]{FEF9F9}-0.1               & \cellcolor[HTML]{FEF9F9}-0.1               \\
\bottomrule
all                        & avg.                         & 81.1                         & 83.0                           & \textbf{83.8}                         & \textbf{83.9}                         & \cellcolor[HTML]{FEFFFF}0.04               & \cellcolor[HTML]{FAFDFB}0.20              
\end{tabular}
\caption{LAS scores on dev sets for \textsc{m} $=$ \textsc{Mono}, \textsc{c} $=$ \textsc{Concat}, \textsc{de} $=$ \textsc{dataemb.-encoder}, \textsc{dd} $=$ \textsc{dataemb.-decoder}.  }
\label{tab:results}
\end{table}%

==> table-2.tex <==
\begin{table}
\centering
\resizebox{.75\textwidth}{!}{
\begin{tabular}{l l r r r r r r}
\toprule
cluster & treebank & self & concat & decoder & encoder & both  & gain \\
\midrule
af-de-nl & UD\_German-GSD & 87.02 & \textbf{87.60} & 87.52 & 87.09 & 87.31 & -0.08 \\
 & UD\_Dutch-LassySmall & 87.25 & 89.71 & \textbf{89.91} & 89.59 & 89.69 & 0.20 \\
 & UD\_Afrikaans-AfriBooms & 80.63 & 82.12 & \textbf{82.62} & 81.17 & 80.93 & 0.50 \\
 & UD\_Dutch-Alpino & 92.75 & 93.01 & 92.97 & 92.50 & \textbf{93.15} & 0.14 \\
\midrule 
e-sla & UD\_Russian-Taiga & 74.93 & 74.54 & 75.11 & 75.75 & \textbf{76.21} & 1.28 \\
 & UD\_Ukrainian-IU & 88.56 & 89.96 & \textbf{89.97} & 89.73 & 89.56 & 0.01 \\
 & UD\_Russian-SynTagRus & \textbf{94.75} & 94.74 & 94.56 & 94.60 & 94.67 & -0.08 \\
\midrule 
en & UD\_English-EWT & 89.34 & 88.90 & 89.06 & \textbf{89.67} & 89.12 & 0.33 \\
 & UD\_English-LinES & 86.57 & 84.72 & 84.77 & 87.00 & \textbf{87.38} & 0.81 \\
 & UD\_English-GUM & 90.38 & 89.06 & 90.17 & 90.74 & \textbf{90.91} & 0.53 \\
\midrule 
es-ca & UD\_Catalan-AnCora & 93.33 & 93.66 & 93.56 & 93.42 & \textbf{93.76} & 0.10 \\
 & UD\_Spanish-AnCora & 92.99 & 93.08 & \textbf{93.38} & 93.30 & 93.30 & 0.30 \\
\midrule 
finno & UD\_North\_Sami-Giella & 49.86 & 62.35 & 62.74 & 62.96 & \textbf{64.71} & 2.36 \\
 & UD\_Estonian-EDT & \textbf{85.61} & 84.66 & 85.29 & 85.11 & 85.33 & -0.28 \\
 & UD\_Finnish-FTB & 89.03 & 82.22 & 89.53 & \textbf{90.14} & 89.87 & 1.11 \\
 & UD\_Finnish-TDT & 88.55 & 82.59 & 88.99 & 88.90 & \textbf{89.35} & 0.81 \\
\midrule 
fr & UD\_French-Spoken & 79.15 & 83.80 & 83.33 & \textbf{84.30} & 83.89 & 0.51 \\
 & UD\_French-GSD & 94.45 & \textbf{94.62} & 94.40 & 94.57 & 94.46 & -0.05 \\
 & UD\_French-Sequoia & 88.55 & 85.85 & 87.86 & \textbf{91.32} & 90.91 & 2.77 \\
\midrule 
indic & UD\_Urdu-UDTB & 81.02 & 81.78 & 81.93 & \textbf{82.01} & 81.74 & 0.23 \\
 & UD\_Hindi-HDTB & 92.54 & 92.47 & 92.56 & \textbf{92.66} & 92.37 & 0.12 \\
\midrule 
iranian & UD\_Persian-Seraji & \textbf{87.01} & 86.96 & 86.84 & 86.37 & 86.28 & -0.17 \\
 & UD\_Kurmanji-MG & 21.43 & 14.29 & 16.67 & \textbf{33.33} & 30.95 & 11.90 \\
\midrule 
it & UD\_Italian-PoSTWITA & 79.66 & 80.00 & \textbf{80.34} & \textbf{80.34} & 80.26 & 0.34 \\
 & UD\_Italian-ISDT & 92.92 & \textbf{93.33} & 93.22 & 92.96 & 93.09 & -0.10 \\
\midrule 
ko & UD\_Korean-GSD & \textbf{82.80} & 71.46 & 79.63 & 82.71 & 82.24 & -0.10 \\
 & UD\_Korean-Kaist & 87.05 & 81.52 & 86.52 & \textbf{87.66} & 87.54 & 0.60 \\
\midrule 
n-ger & UD\_Swedish-LinES & 84.93 & 85.07 & 85.43 & 86.03 & \textbf{86.05} & 0.98 \\
 & UD\_Danish-DDT & 86.24 & 86.37 & 86.32 & \textbf{87.05} & 86.50 & 0.68 \\
 & UD\_Norwegian-NynorskLIA & 74.23 & 76.72 & 77.18 & 76.94 & \textbf{77.26} & 0.54 \\
 & UD\_Swedish-Talbanken & 83.85 & 84.30 & 85.32 & 85.85 & \textbf{85.90} & 1.60 \\
 & UD\_Norwegian-Bokmaal & 93.91 & 94.18 & \textbf{94.77} & 94.31 & 94.26 & 0.59 \\
 & UD\_Norwegian-Nynorsk & 92.57 & 92.85 & 93.21 & \textbf{93.30} & 92.93 & 0.45 \\
\midrule 
old & UD\_Latin-ITTB & 90.08 & 89.98 & \textbf{90.17} & 89.93 & 89.62 & 0.08 \\
 & UD\_Ancient\_Greek-Perseus & 60.48 & \textbf{65.13} & 64.86 & 64.17 & 64.35 & -0.27 \\
 & UD\_Ancient\_Greek-PROIEL & 75.57 & 77.37 & 77.26 & \textbf{77.46} & 76.91 & 0.08 \\
 & UD\_Latin-Perseus & 56.28 & 65.34 & 65.63 & \textbf{70.07} & 69.72 & 4.73 \\
 & UD\_Latin-PROIEL & 77.59 & 79.56 & 79.76 & \textbf{79.99} & 78.84 & 0.43 \\
 & UD\_Old\_Church\_Slavonic-PROIEL & 61.24 & 64.48 & \textbf{65.22} & 64.88 & 63.91 & 0.74 \\
 & UD\_Gothic-PROIEL & 72.74 & 80.36 & \textbf{80.75} & 79.87 & 79.91 & 0.40 \\
\midrule 
pt-gl & UD\_Galician-TreeGal & 70.80 & 65.73 & 75.01 & 81.07 & \textbf{82.11} & 11.31 \\
 & UD\_Portuguese-Bosque & 90.45 & 90.41 & 90.43 & 90.52 & \textbf{90.62} & 0.17 \\
 & UD\_Galician-CTG & 81.16 & 80.92 & 80.94 & \textbf{81.70} & 81.38 & 0.54 \\
\midrule 
sw-sla & UD\_Croatian-SET & 88.20 & 88.33 & \textbf{88.43} & 88.39 & 88.17 & 0.10 \\
 & UD\_Serbian-SET & 87.20 & 87.78 & 88.89 & \textbf{88.94} & 88.88 & 1.16 \\
 & UD\_Slovenian-SST & 60.30 & 70.67 & \textbf{70.78} & 70.40 & 70.28 & 0.11 \\
 & UD\_Slovenian-SSJ & 93.22 & \textbf{93.54} & 93.29 & 93.39 & 93.44 & -0.09 \\
\midrule 
turkic & UD\_Turkish-IMST & 65.57 & \textbf{66.02} & 65.66 & 64.48 & 64.86 & -0.35 \\
 & UD\_Buryat-BDT & 19.51 & 26.83 & 31.71 & \textbf{36.59} & 21.95 & 9.76 \\
 & UD\_Uyghur-UDT & 47.85 & 49.11 & 49.01 & \textbf{49.18} & 48.68 & 0.07 \\
 & UD\_Kazakh-KTB & 14.02 & \textbf{62.62} & 58.88 & 48.60 & 49.53 & -3.74 \\
\midrule 
w-sla & UD\_Czech-FicTree & 92.97 & 94.01 & 94.23 & 94.23 & \textbf{94.41} & 0.40 \\
 & UD\_Czech-CAC & 91.86 & \textbf{92.24} & 92.19 & 92.20 & 92.18 & -0.05 \\
 & UD\_Upper\_Sorbian-UFAL & 14.47 & 59.21 & 60.53 & \textbf{63.16} & 59.21 & 3.95 \\
 & UD\_Czech-PDT & 89.57 & 90.39 & \textbf{90.57} & 90.45 & 90.42 & 0.18 \\
 & UD\_Slovak-SNK & 92.07 & 93.62 & 93.51 & \textbf{93.77} & 93.58 & 0.14 \\
 & UD\_Polish-LFG & 95.41 & 93.30 & 96.17 & \textbf{96.49} & 96.40 & 1.08 \\
 & UD\_Polish-PDB & 91.64 & 91.29 & \textbf{91.82} & 91.72 & 91.72 & 0.18 \\
\midrule
 & avg. & 78.52 & 80.63 & 81.58 & \textbf{82.16} & 81.77 & 1.04 \\
\bottomrule
\end{tabular}}
\caption{}
\label{tab:results}
\end{table}

==> table-3.tex <==
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{.7}
\resizebox{.92\textwidth}{!}{
\begin{tabular}{l l |c |cccc |cccc }
\toprule
& & & \multicolumn{4}{c|}{Trained on clusters} & \multicolumn{4}{c}{Trained on all}\\
\midrule
Cluster & Treebank & \textsc{mono} & \textsc{concat} & \textsc{decoder} & \textsc{encoder} & \textsc{both} & \textsc{concat} & \textsc{decoder} & \textsc{encoder} & \textsc{both} \\
\midrule 
af-de-nl & af\_afribooms & 80.63 & 82.12 & \textbf{82.62} & 81.17 & 80.93 & 82.98 & \textbf{83.53} & 82.62 & 82.37 \\
 & nl\_alpino & 92.75 & 93.01 & 92.97 & 92.50 & \textbf{93.15} & 92.65 & 92.59 & \textbf{93.08} & 92.76 \\
 & nl\_lassysmall & 87.25 & 89.71 & \textbf{89.91} & 89.59 & 89.69 & 89.45 & \textbf{90.29} & 90.11 & 90.05 \\
 & de\_gsd & 87.02 & \textbf{87.60} & 87.52 & 87.09 & 87.31 & 87.63 & \textbf{87.63} & 87.25 & 87.53 \\
\midrule 
e-sla & ru\_syntagrus & \textbf{94.75} & 94.74 & 94.56 & 94.60 & 94.67 & 94.50 & 94.45 & 94.51 & 94.52 \\
 & ru\_taiga & 74.93 & 74.54 & 75.11 & 75.75 & \textbf{76.21} & 75.43 & 75.95 & \textbf{76.46} & 76.45 \\
 & uk\_iu & 88.56 & 89.96 & \textbf{89.97} & 89.73 & 89.56 & 90.28 & \textbf{90.67} & 90.58 & 90.26 \\
\midrule 
en & en\_ewt & 89.34 & 88.90 & 89.06 & \textbf{89.67} & 89.12 & 88.49 & 88.16 & 88.86 & \textbf{88.94} \\
 & en\_gum & 90.38 & 89.06 & 90.17 & 90.74 & \textbf{90.91} & 88.64 & 89.65 & 90.53 & \textbf{90.71} \\
 & en\_lines & 86.57 & 84.72 & 84.77 & 87.00 & \textbf{87.38} & 84.70 & 85.08 & 87.41 & \textbf{87.42} \\
\midrule 
es-ca & ca\_ancora & 93.33 & 93.66 & 93.56 & 93.42 & \textbf{93.76} & 93.45 & 93.43 & \textbf{93.46} & 93.44 \\
 & es\_ancora & 92.99 & 93.08 & \textbf{93.38} & 93.30 & 93.30 & \textbf{93.35} & 93.28 & 93.24 & 93.16 \\
\midrule 
finno & et\_edt & \textbf{85.61} & 84.66 & 85.29 & 85.11 & 85.33 & 85.17 & 84.98 & 85.58 & 85.58 \\
 & fi\_ftb & 89.03 & 82.22 & 89.53 & \textbf{90.14} & 89.87 & 80.15 & 89.01 & 89.06 & \textbf{89.38} \\
 & fi\_tdt & 88.55 & 82.59 & 88.99 & 88.90 & \textbf{89.35} & 84.24 & 89.13 & \textbf{89.44} & 89.39 \\
 & sme\_giella$^*$ & 49.86 & 62.35 & 62.74 & 62.96 & \textbf{64.71} & 59.55 & 59.55 & 63.95 & \textbf{65.28} \\
\midrule 
fr & fr\_gsd & 94.45 & \textbf{94.62} & 94.40 & 94.57 & 94.46 & 94.49 & 94.42 & 94.44 & \textbf{94.54} \\
 & fr\_sequoia & 88.55 & 85.85 & 87.86 & \textbf{91.32} & 90.91 & 86.17 & 86.46 & 91.68 & \textbf{91.73} \\
 & fr\_spoken & 79.15 & 83.80 & 83.33 & \textbf{84.30} & 83.89 & 83.47 & 83.20 & 84.09 & \textbf{84.50} \\
\midrule 
indic & hi\_hdtb & 92.54 & 92.47 & 92.56 & \textbf{92.66} & 92.37 & 92.49 & 92.37 & \textbf{92.51} & 92.34 \\
 & ur\_udtb & 81.02 & 81.78 & 81.93 & \textbf{82.01} & 81.74 & 81.66 & 81.41 & \textbf{81.77} & 81.42 \\
\midrule 
iranian & kmr\_mg$^*$ & 21.43 & 14.29 & 16.67 & \textbf{33.33} & 30.95 & 21.43 & 19.05 & \textbf{28.57} & 14.29 \\
 & fa\_seraji & \textbf{87.01} & 86.96 & 86.84 & 86.37 & 86.28 & 86.32 & 86.30 & 86.54 & 86.27 \\
\midrule 
it & it\_isdt & 92.92 & \textbf{93.33} & 93.22 & 92.96 & 93.09 & \textbf{93.44} & 93.26 & 93.24 & 93.29 \\
 & it\_postwita & 79.66 & 80.00 & \textbf{80.34} & \textbf{80.34} & 80.26 & 79.96 & 80.08 & \textbf{80.72} & 80.16 \\
\midrule 
ko & ko\_gsd & \textbf{82.80} & 71.46 & 79.63 & 82.71 & 82.24 & 69.41 & 79.13 & 82.55 & 82.77 \\
 & ko\_kaist & 87.05 & 81.52 & 86.52 & \textbf{87.66} & 87.54 & 81.12 & 85.81 & \textbf{87.07} & 86.86 \\
\midrule 
n-ger & da\_ddt & 86.24 & 86.37 & 86.32 & \textbf{87.05} & 86.50 & 85.90 & 85.30 & \textbf{86.41} & 86.31 \\
 & no\_bokmaal & 93.91 & 94.18 & \textbf{94.77} & 94.31 & 94.26 & 94.17 & 94.28 & 94.15 & \textbf{94.30} \\
 & no\_nynorsk & 92.57 & 92.85 & 93.21 & \textbf{93.30} & 92.93 & 92.73 & 92.47 & 92.93 & \textbf{93.15} \\
 & no\_nynorsklia & 74.23 & 76.72 & 77.18 & 76.94 & \textbf{77.26} & 76.76 & 76.85 & \textbf{77.39} & 77.18 \\
 & sv\_lines & 84.93 & 85.07 & 85.43 & 86.03 & \textbf{86.05} & 85.15 & 85.30 & \textbf{86.19} & \textbf{86.19} \\
 & sv\_talbanken & 83.85 & 84.30 & 85.32 & 85.85 & \textbf{85.90} & 85.18 & 85.41 & \textbf{86.64} & 86.14 \\
\midrule 
old & grc\_proiel$^*$ & 75.57 & 77.37 & 77.26 & \textbf{77.46} & 76.91 & \textbf{76.76} & 76.70 & 76.30 & 76.47 \\
 & grc\_perseus$^*$ & 60.48 & \textbf{65.13} & 64.86 & 64.17 & 64.35 & \textbf{64.52} & 64.41 & 63.93 & 64.29 \\
 & got\_proiel$^*$ & 72.74 & 80.36 & \textbf{80.75} & 79.87 & 79.91 & 78.97 & 78.72 & 78.72 & \textbf{79.50} \\
 & la\_ittb & 90.08 & 89.98 & \textbf{90.17} & 89.93 & 89.62 & \textbf{90.30} & 90.13 & 90.08 & 90.16 \\
 & la\_proiel & 77.59 & 79.56 & 79.76 & \textbf{79.99} & 78.84 & 79.07 & 78.96 & \textbf{79.41} & 79.13 \\
 & la\_perseus & 56.28 & 65.34 & 65.63 & \textbf{70.07} & 69.72 & 64.71 & 65.40 & \textbf{71.56} & 70.05 \\
 & cu\_proiel$^*$ & 61.24 & 64.48 & \textbf{65.22} & 64.88 & 63.91 & 64.11 & 64.42 & 64.17 & \textbf{64.93} \\
\midrule 
pt-gl & gl\_ctg & 81.16 & 80.92 & 80.94 & \textbf{81.70} & 81.38 & 80.93 & 80.89 & 81.50 & \textbf{81.56} \\
 & gl\_treegal & 70.80 & 65.73 & 75.01 & 81.07 & \textbf{82.11} & 64.60 & 68.93 & \textbf{82.49} & 82.28 \\
 & pt\_bosque & 90.45 & 90.41 & 90.43 & 90.52 & \textbf{90.62} & \textbf{90.49} & 90.28 & 90.44 & 90.09 \\
\midrule 
sw-sla & hr\_set & 88.20 & 88.33 & \textbf{88.43} & 88.39 & 88.17 & 88.35 & 88.73 & \textbf{88.84} & 88.74 \\
 & sr\_set & 87.20 & 87.78 & 88.89 & \textbf{88.94} & 88.88 & 88.31 & 89.16 & 89.47 & \textbf{89.48} \\
 & sl\_ssj & 93.22 & \textbf{93.54} & 93.29 & 93.39 & 93.44 & 93.37 & 93.30 & \textbf{93.40} & 93.29 \\
 & sl\_sst & 60.30 & 70.67 & \textbf{70.78} & 70.40 & 70.28 & 70.31 & 70.84 & \textbf{71.22} & 71.09 \\
\midrule 
turkic & bxr\_bdt$^*$ & 19.51 & 26.83 & 31.71 & \textbf{36.59} & 21.95 & 26.83 & 21.95 & 29.27 & \textbf{31.71} \\
 & kk\_ktb & 14.02 & \textbf{62.62} & 58.88 & 48.60 & 49.53 & 59.81 & \textbf{61.68} & 51.40 & 49.53 \\
 & tr\_imst & 65.57 & \textbf{66.02} & 65.66 & 64.48 & 64.86 & \textbf{66.29} & 66.03 & 65.99 & 66.00 \\
 & ug\_udt$^*$ & 47.85 & 49.11 & 49.01 & \textbf{49.18} & 48.68 & \textbf{50.39} & 49.86 & 50.06 & 49.91 \\
\midrule 
w-sla & cs\_cac & 91.86 & \textbf{92.24} & 92.19 & 92.20 & 92.18 & 92.12 & 92.22 & 92.09 & \textbf{92.40} \\
 & cs\_fictree & 92.97 & 94.01 & 94.23 & 94.23 & \textbf{94.41} & 94.11 & 94.35 & \textbf{94.52} & 94.10 \\
 & cs\_pdt & 89.57 & 90.39 & \textbf{90.57} & 90.45 & 90.42 & 90.32 & 90.34 & 90.89 & \textbf{90.89} \\
 & pl\_lfg & 95.41 & 93.30 & 96.17 & \textbf{96.49} & 96.40 & 92.87 & 96.19 & \textbf{96.43} & \textbf{96.43} \\
 & pl\_pdb & 91.64 & 91.29 & \textbf{91.82} & 91.72 & 91.72 & 91.74 & 91.85 & 91.72 & \textbf{91.94} \\
 & sk\_snk & 92.07 & 93.62 & 93.51 & \textbf{93.77} & 93.58 & 93.13 & \textbf{93.41} & 93.29 & 93.02 \\
 & hsb\_ufal$^*$ & 14.47 & 59.21 & 60.53 & \textbf{63.16} & 59.21 & 61.84 & \textbf{65.79} & 61.84 & 63.16 \\
\midrule
 & avg. & 78.52 & 80.63 & 81.58 & \textbf{82.16} & 81.77 & 80.60 & 81.26 & \textbf{82.10} & 81.88 \\
\bottomrule
\end{tabular}}
\caption{LAS scores for each dataset (dev) for all of our settings, both when training a parser per cluster (``Trained on cluster''), as well as having one parser for all treebanks (``Trained on all''). Bold: highest score for this training setup, omitted if the \textsc{mono} baseline performs best. $^*$ not used in mBERT pretraining.}
\label{tab:results}
\end{table}
